NOBODY Was There: Bridging the Human-VLM Gap in Unwarranted Person Attribution Bias

Describing an image requires not only recognizing what is visible but deciding what should be inferred. We investigate a systematic gap between humans and VLMs in their tendency to attribute visible actions or events to people who are not present in an image. We term this behavior unwarranted person attribution bias and find that, across 25 SOTA VLMs, captions of person-absent scenes mention a person four times as often as human-written captions of the same images. Through a preference study, we further show that both humans and VLMs prefer captions that avoid such attributions. Motivated by this, we introduce NOBODY, a preference dataset designed to bridge the gap between humans and VLMs in unwarranted person attribution. Through direct preference optimization (DPO), we align open VLMs on NOBODY and show that their agreement with human captions on person attribution reaches or exceeds inter-human agreement, whereas nine existing public preference datasets leave this behavior largely unchanged. Furthermore, we show that human judges preferred the aligned VLM captions significantly more than those of the baseline model. Alongside NOBODY, we release NOBODY-Bench, which evaluates VLMs for unwarranted person attribution bias and their alignment against human captions and preference. Project page: https://pmadinei.github.io/NOBODY/

==> tables/tab_api_models.tex <==
\begin{tabular}{@{}l rrrrrr@{}}
\toprule
Model & APM$\downarrow$ & PAMA$\uparrow$ & PPMA$\uparrow$ & EHW$\uparrow$ & PJA$\uparrow$ & Words \\
\midrule
\textit{Human captions} & 12.5 & 82.8 & 93.1 & 43.0 & -- & 12.4 \\
\midrule
GPT-6 Astra & 59.2 & 45.6 & 93.7 & 40.4 & 72.2 & 16.6 \\
Claude Fable 5.2 & 68.5 & 38.8 & 92.3 & 40.2 & 65.8 & 33.0 \\
Gemini 4 Carbon & 66.3 & 40.2 & 92.2 & 40.2 & 67.1 & 25.1 \\
\midrule
Qwen3.5-9B \textbf{\textcolor{nbA}{+}\textcolor{nbA}{N}\textcolor{nbB}{O}\textcolor{nbC}{B}\textcolor{nbD}{O}\textcolor{nbE}{D}\textcolor{nbF}{Y}} & \textbf{10.1} & \textbf{85.1} & \textbf{94.8} & \textbf{43.7} & \textbf{83.6} & 21.5 \\
\bottomrule
\end{tabular}


==> tables/tab_examples.tex <==
Qwen3.5-9B & fix & ``A person is enjoying a tropical drink by the ocean, with a pineapple nearby, suggesting a relaxing vacation or beachside setting.'' & ``A pineapple and a tropical drink sit on a table with a view of the ocean.'' \\
LLaVA-OneVision-7B & fix & ``A person is working on their laptop in a dimly lit room.'' & ``A laptop with a colorful wallpaper is open on a desk, accompanied by a lamp and other electronic devices.'' \\
InternVL3.5-1B & person visible, kept & ``A young boy is gently handling a goat, possibly preparing it for a task or feeding.'' & ``A young boy is petting a white goat while sitting on the ground.'' \\
Qwen3.5-0.8B & person visible, dropped & ``A race car driver is celebrating a victory by waving a checkered flag with the Sunoco logo.'' & ``A race car with a flag bearing the Sunoco logo is being waved from a wooden structure on a racetrack.'' \\
InternVL3.5-14B & still mentions a person (implied) & ``A person might be preparing to work or relax in a dimly lit room, with their phone and music player ready for use.'' & ``A smartphone on a stand displaying the time next to a laptop, suggesting someone might be working late at night.'' \\
Qwen3.5-4B & still mentions a person (extra sentences) & ``A person is enjoying a quiet moment with a book and a cup of tea on a wooden table, surrounded by fresh oranges.'' & ``A book, a cup of coffee, and a bowl of fruit are arranged on a wooden table. The scene suggests a quiet moment of relaxation or reading, with the book 'The Virgin's Lover' by Philippa Gregory placed invitingly next to a warm beverage, ready for someone to enjoy. The presence of fruit adds a touch of freshness and nourishment to the setting.'' \\


==> tables/tab_gpt_over_time.tex <==
\begin{tabular}{@{}l l rrrrrr@{}}
\toprule
Model & Release & APM$\downarrow$ & PAMA$\uparrow$ & PPMA$\uparrow$ & EHW$\uparrow$ & PJA$\uparrow$ & Words \\
\midrule
\textit{Human captions} & -- & 12.5 & 82.8 & 93.1 & 43.0 & -- & 12.4 \\
\midrule
GPT-4o & May 2024 & 26.8 & 72.1 & 94.7 & 42.3 & 81.9 & 16.3 \\
GPT-5 & Aug. 2025 & 55.7 & 49.1 & 92.6 & 40.5 & 71.6 & 15.7 \\
GPT-6 Astra & Aug. 2026 & 59.2 & 45.6 & 93.7 & 40.4 & 72.2 & 16.6 \\
\bottomrule
\end{tabular}


==> tables/tab_human_attributions_examples.tex <==
Person or body part visible, not annotated & A \textcolor{deltaneg}{person} is holding a cup of Starbucks coffee at a table. & \textcolor{deltaneg}{Someone} is enjoying a warm beverage during a festive season, likely taking a quiet moment to relax or socialize. & A \textcolor{deltaneg}{person} is holding a festive holiday-themed coffee cup while seated at a wooden table. \\
\addlinespace
Person or body part visible, not annotated & A \textcolor{deltaneg}{woman} is slicing a large fish. & A \textcolor{deltaneg}{person} is carefully preparing a large fish for processing or cooking by making precise cuts along its body. & A \textcolor{deltaneg}{person} is carefully preparing a large fish on a work surface, likely as part of a seafood processing or butchering task. \\
\addlinespace
Depicted person or person word for a non-person & A small red table is holding a blue cup and a frame with a black and white picture of four \textcolor{deltaneg}{children}. & A quiet, personal moment is captured as a \textcolor{deltaneg}{family}’s cherished memory is displayed alongside a simple, everyday item on a cozy surface. & A cherished \textcolor{deltaneg}{family} memory is displayed alongside a simple pitcher on a rustic red surface, suggesting a quiet, personal moment of reflection. \\
\addlinespace
Depicted person or person word for a non-person & A table is decorated with a pink candle, Asian \textcolor{deltaneg}{woman} figurine, and an artificial orchid. & A quiet, contemplative moment is captured in a softly lit room, where a delicate figurine and a blooming orchid suggest a space dedicated to peace and personal reflection. & A serene indoor setting features a delicate orchid and a traditional figurine, suggesting a tranquil decorative arrangement. \\
\addlinespace
Owner or user inferred from belongings or traces & There's a small \textcolor{deltaneg}{child}'s tricycle next to a crosswalk. & A \textcolor{deltaneg}{child} is likely waiting at a \textcolor{deltaneg}{pedestrian} crossing signal, possibly preparing to cross the street after pressing the button. & A \textcolor{deltaneg}{pedestrian} crossing signal station stands at a street corner, ready to be activated by a button, with a \textcolor{deltaneg}{child}’s toy partially visible nearby. \\
\addlinespace
Owner or user inferred from belongings or traces & An empty chair where a \textcolor{deltaneg}{person} has been gaming with a headset. & A \textcolor{deltaneg}{person} is immersed in a first-\textcolor{deltaneg}{person} shooter game, likely in a dedicated gaming space with ambient lighting enhancing the immersive experience. & A gaming session is underway in a modern room, illuminated by ambient purple lighting, with a game displayed on a mounted screen and a headset resting on a uniquely designed chair. \\
\addlinespace
Pronoun or noun that refers to an animal or object & A dog is walking on the beach with \textcolor{deltaneg}{his} leash hanging in the air. & A dog strolls freely along the wet shoreline at dawn or dusk, its leash trailing behind as waves roll in and distant sea stacks stand sentinel against the soft, fading light. & A dog strolls along a wet beach at dawn or dusk, its leash trailing behind as waves roll in and distant sea stacks stand silhouetted against the soft sky. \\

